On the Descriptional Complexity of Operations on Semilinear Sets

We investigate the descriptional complexity of operations on semilinear sets. Roughly speaking, a semilinear set is the finite union of linear sets, which are built by constant and period vectors. The interesting parameters of a semilinear set are: (i) the maximal value that appears in the vectors of periods and constants and (ii) the number of such sets of periods and constants necessary to describe the semilinear set under consideration. More precisely, we prove upper bounds on the union, intersection, complementation, and inverse homomorphism. In particular, our result on the complementation upper bound answers an open problem from [G. J. LAVADO, G. PIGHIZZINI, S. SEKI: Operational State Complexity of Parikh Equivalence, 2014].

==> eptcsdata.tex <==
\providecommand{\firstpage}{41}
\providecommand{\publicationstatus}{E. Csuhaj-Varj\'u, P. D\"om\"osi, Gy. Vaszil (Eds.): 15th International \\ Conference on Automata and Formal Languages (AFL 2017)\\
EPTCS 252, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.252.8}{10.4204/EPTCS.252.8}}

